Improving Performance of Object Detection using the Mechanisms of Visual Recognition in Humans

Object recognition systems are usually trained and evaluated on high resolution images. However, in real world applications, it is common that the images have low resolutions or have small sizes. In this study, we first track the performance of the state-of-the-art deep object recognition network, Faster- RCNN, as a function of image resolution. The results reveals negative effects of low resolution images on recognition performance. They also show that different spatial frequencies convey different information about the objects in recognition process. It means multi-resolution recognition system can provides better insight into optimal selection of features that results in better recognition of objects. This is similar to the mechanisms of the human visual systems that are able to implement multi-scale representation of a visual scene simultaneously. Then, we propose a multi-resolution object recognition framework rather than a single-resolution network. The proposed framework is evaluated on the PASCAL VOC2007 database. The experimental results show the performance of our adapted multi-resolution Faster-RCNN framework outperforms the single-resolution Faster-RCNN on input images with various resolutions with an increase in the mean Average Precision (mAP) of 9.14% across all resolutions and 1.2% on the full-spectrum images. Furthermore, the proposed model yields robustness of the performance over a wide range of spatial frequencies.

==> sections/Training.tex <==
\section{Training Faster-RCNN on Multiple Resolutions}

We train the Faster-RCNN network on 5 resolution levels including $R_{5}, R_{10}, R_{18}, R_{20}$, and full-spectrum using the corresponding datasets (PASCAL VOC2007-$R_{5, 10, 18, 20}$)
that were described in the previous subsection. Each dataset provides the training and test images in different levels of resolution. For example, the PASCAL VOC2007-$R_5$ database is obtained by applying a Gaussian blur to the original PASCAL VOC2007 image database. A cut off frequency of 0.25$w$ ($w$ is the longer side of the images) is considered for a 2D Gaussian filter in the frequency domain. This systematic change of resolution from low to high is to ensure that the Faster-RCNN can maintain good performance on all spatial frequencies. The trained models are called Full-spectrum Model, $\frac{20}{20}$-Model, $\frac{18}{20}$-Model, $\frac{10}{20}$ -Model, and $\frac{5}{20}$-Model, each being trained with images in a specific resolution level.

We test the models on the test dataset (4952) in all resolution levels (21 levels) for
all 20 object classes and report the performance by the mAP values for each level of resolution. Testing models on images of all resolution levels has the advantage that it will reveal the range of frequencies that each model is sensitive to and functions efficiently.

Table \ref{tb:Performance comparison} summarizes the mAP(\%) values for the 5 models on 5 test datasets in 5 different resolutions. The results indicate that: 1) Models that are trained in a slightly lower resolution ($R_{18}$ and $R_{20}$) outperform the Full-spectrum Model on input images with various degrees of resolutions from the full-spectrum images to very low resolution images. Even the $\frac{18}{20}$- Model outperforms the $\frac{20}{20}$- Model in full and very high resolution images.

Figure \ref{fig:The detection power} illustrates a sample full-resolution image that
has been tested on different resolution models. The result of the object recognition process shows that the second person in the image (shown with yellow bounding box) that had not been detected by the Full-spectrum Model and the $\frac{20}{20}$- Model can be detected by the $\frac{18}{20}$ - Model and the $\frac{10}{20}$ - Model. That is, these models can generalize wider range of frequencies than the Full-spectrum Model. For example, an mAP for the Full-spectrum Model drops from 68.1\% to 60.1\% when exposing to the images with low resolution of $R_{10}$. However, for the same resolution input images, an mAP in the $\frac{18}{20}$- Model only changes from 68.4\% to 65.3\% (more robust performance). 2) Models that are trained on the low resolution images ($R_{10}$ and $R_5$) exhibit significant, robust improvement in recognition of low resolution images. 3) Combining multiple models in different resolutions not only improves the performance but also the robustness against the resolution level of the input images. Then, in the combined model, there is no need to determine the frequency range of the input image and pass it to an appropriate model. Hence, similar to the human visual system, we propose a multi-resolution Faster-RCNN model that provides robust and high recognition performance regardless of the resolution of the input images. 
%The next section describes the model and provides a detailed performance evaluation on images of all degrees of resolution.

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.48\textwidth]{figures/fig9.jpg}
\end{center}
\caption{The detection power of Faster-RCNN networks trained in different resolutions for recognition of objects in a sample image.}
\label{fig:The detection power}
\end{figure}



